E(n) Equivariant Graph Neural Networks

This paper introduces a new model to learn graph neural networks equivariant to rotations, translations, reflections and permutations called E(n)-Equivariant Graph Neural Networks (EGNNs). In contrast with existing methods, our work does not require computationally expensive higher-order representations in intermediate layers while it still achieves competitive or better performance. In addition, whereas existing methods are limited to equivariance on 3 dimensional spaces, our model is easily scaled to higher-dimensional spaces. We demonstrate the effectiveness of our method on dynamical systems modelling, representation learning in graph autoencoders and predicting molecular properties.

==> E(n) Equivariant Graph Neural Networks _ ICML 2021/sections/background.tex <==

\section{Background}
In this section we introduce the relevant materials on equivariance and graph neural networks which will later complement the definition of our method.

\subsection{Equivariance}
\label{sec:background_equivariance}
Let $T_g: X \xrightarrow{} X$ be a set of transformations on $X$ for the abstract group $g \in G$. We say a function $\phi: X \xrightarrow{} Y$ is equivariant to $g$ if there exists an equivalent transformation on its output space $S_g: Y \xrightarrow{} Y$  such that:
\begin{equation} \label{eq:equivariance}
    \phi(T_g(\rmx)) = S_g(\phi(\rmx)) 
\end{equation}
As a practical example, let $\phi(\cdot)$ be a non-linear function, $\rmx = (\rmx_1, \dots, \rmx_M) \in \mathbb{R}^{M \times n}$ an input set of $M$ point clouds embedded in a $n$-dimensional space, $\phi(\rmx) = \rmy \in \mathbb{R}^{M \times n}$ the transformed set of point clouds, $T_g$ a translation on the input set $T_g(\rmx) = \rmx + g$ and $S_g$ an equivalent translation on the output set $S_g(\rmy) = \rmy + g$. If our transformation $\phi: X \xrightarrow{} Y$ is translation equivariant, translating the input set $T_g(\rmx)$ and then applying the function $\phi(T_x(\rmx))$ on it, will deliver the same result as first running the function $y=\phi(\rmx)$ and then applying an equivalent translation to the output $T_g(\rmy)$ such that Equation \ref{eq:equivariance} is fulfilled and $\phi(\rmx + g) = \phi(\rmx) + g$. In this work we explore the following three types of equivariance on a set of particles $\rmx$:
\begin{enumerate}[nolistsep]
    \item Translation equivariance. Translating the input by $g \in \mathbb{R}^n$ results in an equivalent translation of the output. Let $\rmx + g$ be shorthand for $(\rmx_1 + g, \ldots, \rmx_M + g)$. Then $\rmy + g = \phi(\rmx + g)$ 
    \item Rotation (and reflection) equivariance. For any orthogonal matrix $Q \in \mathbb{R}^{n \times n}$, let $Q\rmx$ be shorthand for $(Q\rmx_1, \ldots, Q\rmx_M)$. Then rotating the input results in an equivalent rotation of the output $Q\rmy = \phi(Q\rmx)$.
    \item Permutation equivariance. Permuting the input results in the same permutation of the output $P(\rmy) = \phi(P(\rmx))$ where $P$ is a permutation on the row indexes.
\end{enumerate}

Note that velocities $\rmv 
\in \mathbb{R}^{M \times n}$ are unaffected by translations, but they transform equivalently under rotation (2) and permutation~(3). Our method introduced in Section \ref{sec:method_main} will satisfy the three above mentioned equivariant constraints. 

\subsection{Graph Neural Networks}
\label{sec:background_gnn}
Graph Neural Networks are permutation equivariant networks that operate on graph structured data \cite{bruna2013spectral, defferrard2016convolutional, kipf2016semi}. Given a graph $\mathcal{G} = (\mathcal{V}, \mathcal{E})$ with nodes $v_i \in \mathcal{V}$ and edges $e_{ij} \in \mathcal{E}$ we define a graph convolutional layer following notation from \cite{gilmer2017neural} as:

\begin{equation} \label{eq:gnn}
\begin{aligned}
\rmm_{ij} &= \phi_e(\rmh_i^l, \rmh_j^l, a_{ij}) \\
    \rmm_i &= \sum_{j \in \mathcal{N}(i)} \rmm_{i j} \\
    \rmh_i^{l+1} &= \phi_h(\rmh_i^l, \rmm_i) \\
\end{aligned}
\end{equation}

Where $\rmh_i^l \in \mathbb{R}^{\text{nf}}$ is the nf-dimensional embedding of node $v_i$ at layer $l$. $a_{ij}$ are the edge attributes. $\mathcal{N}(i)$ represents the set of neighbors of node $v_i$. Finally, $\phi_e$ and $\phi_h$ are the edge and node operations respectively which are commonly approximated by Multilayer Perceptrons (MLPs).

==> E(n) Equivariant Graph Neural Networks _ ICML 2021/sections/conclusions.tex <==
\section{Conclusions}
Equivariant graph neural networks are receiving increasing interest from the natural and medical sciences as they represent a new tool for analyzing molecules and their properties. In this work, we presented a new $\En$ equivariant deep architecture for graphs that is computationally efficient, easy to implement, and significantly improves over the current state-of-the-art on a wide range of tasks. We believe these properties make it ideally suited to make a direct impact on topics such as drug discovery, protein folding and the design of new materials, as well as applications in 3D computer vision.

\section*{Acknowledgements}
We would like to thank Patrick Forr\'e for his support to formalize the invariance features identification proof. 

%It is simpler and cheaper than some previous methods in that it does not require spherical harmonics and it can facilely be implemented as an extension to the already existing Graph Neural Networks framework. In addition, our method reported competitive or state of the art results in all the conducted experiments.

%We believe translation and rotation equivariant models will play a very important role in the future in a variety of fields. Molecule and graph generation may benefit from it in the near future which can have a direct impact in the chemistry industry (e.g. drug discovery, protein folding). Other fields like physics modelling or 3D point cloud representation may also benefit from it. 

%{\color{blue}[Victor] Here I was thinking to add something "We think that providing a simple and efficient model is key and can have and impact to the community...", but I am not sure how to phrase it or whether to add it or not.}


==> E(n) Equivariant Graph Neural Networks _ ICML 2021/sections/experiments.tex <==
%\section{Potential scenarios where our method can be useful}

%\textbf{N-body Simulations:} This experiment is introduced in \cite{kipf2018neural} and adapted in \cite{fuchs2020se}. N-particles embedded in a 3-dimensional with either negative or positive charge exert repulsive or attractive forces on each other. The algorithm has to predict the relative position of these particles after a given number of time steps. Since the relative positions are invariant to rotations and translations on set of particles our algorithm can benefit from it. The relative position of the particles would be the $X$ coordinates in our algorithm. For more information about the dataset refer to Experiment 4.1 in \cite{fuchs2020se}. 

%\textbf{QM9:} QM9 is a \cite{ramakrishnan2014quantum} publicly available chemical property prediction dataset for molecules with up to 29 atoms per molecule. The position of each atom is provided in the dataset. The atom positions would be the coordinates $X$ in our algorithm. Other molecule datasets where our algorithm could be used are MD17 \cite{chmiela2017machine} and ISO17 \url{http://www.quantum-machine.org/}.


%\textbf{Graph Autoencoder:} In the next section we show how our algorithm can also be used for graph autoencoding. We can randomly assign a n-dimensional particle to each node of the graph and then express the edges of our graph as a similarity measure on pairs of particles. Following this approach we show how our a graph autoencoder built from our equivariant equations overcomes other algorithms when embedding and reconstructing a graph into a low dimensional space. 




%\textbf{Graph Visualization:} Comparison to T-SNE.

%\textbf{Protein folding:} Generating 3D shape proteins from its sequence \cite{eismann2020protein}. As done in Alpha Fold or this workshop paper from NeurIPS \cite{eismann2020protein} uses Tensor Field Networks to generate the 3D shape of a protein beucase they are translation and rotation equivariant.



%\textbf{Limitations:} Experiment 5.1 from Tensor Field Networks \cite{thomas2018tensor} would be the only limitation.  (Pending to explain why).


\section{Experiments}

\subsection{Modelling a dynamical system | N-body system } \label{sec:experiment_n_body}

In a dynamical system a function defines the time dependence of a point or set of points in a geometrical space. Modelling these complex dynamics is crucial in a variety of applications such as control systems \cite{chua2018deep}, model based dynamics in reinforcement learning \cite{nagabandi2018neural}, and physical systems simulations \cite{grzeszczuk1998neuroanimator, watters2017visual}. In this experiment we forecast the positions for a set of particles which are modelled by simple interaction rules, yet can exhibit complex dynamics.

Similarly to \cite{fuchs2020se}, we extended the Charged Particles N-body experiment from \cite{kipf2018neural} to a 3 dimensional space. The system consists of 5 particles that carry a positive or negative charge and have a position and a velocity associated in 3-dimensional space. The system is controlled by physic rules: particles are attracted or repelled depending on their charges. This is an equivariant task since rotations and translations on the input set of particles result in the same transformations throughout the entire trajectory. 


\textbf{Dataset}: We sampled 3.000 trajectories for training, 2.000 for validation and 2.000 for testing. Each trajectory has a duration of 1.000 timesteps. For each trajectory we are provided with the initial particle positions $\rmp^{(0)}=\{ \rmp^{(0)}_1, \dots \rmp^{(0)}_5 \} \in \mathbb{R}^{5 \times 3}$, their initial velocities $\rmv^{(0)}=\{ \rmv^{(0)}_1, \dots \rmv^{(0)}_5 \} \in \mathbb{R}^{5 \times 3}$ and their respective charges $\mathbf{c} = \{c_1, \dots c_5\} \in \{-1, 1\}^5$. The task is to estimate the positions of the five particles after 1.000 timesteps. We optimize the averaged Mean Squared Error of the estimated position with the ground truth one.


\textbf{Implementation details:} In this experiment we used the extension of our model that includes velocity from section \ref{sec:method_velocity}. We input the position $\rmp^{(0)}$ as the first layer coordinates $\rmx^0$ of our model and the velocity $\rmv^{(0)}$ as the initial velocity in Equation \ref{eq:egnn_velocity}, the norms $\|\rmv_i^{(0)} \|$ are also provided as features to $\rmh_i^0$ through a linear mapping. The charges are input as edge attributes $a_{ij} = c_i c_j$. The model outputs the last layer coordinates $\rmx^L$ as the estimated positions.
%We used 4 layers in our EGNN and 64 features for the hidden layers. As non-linearity we used the Swish activation function \cite{ramachandran2017searching}. 
We compare our method to its non equivariant Graph Neural Network (GNN) cousin, and the equivariant methods: Radial Field \cite{kohler2019equivariant_workshop}, Tensor Field Networks and the SE(3) Transformer. All algorithms are composed of 4 layers and have been trained under the same conditions, batch size 100, 10.000 epochs, Adam optimizer, the learning rate was tuned independently for each model. We used 64 features for the hidden layers in the Radial Field, the GNN and our EGNN. As non-linearity we used the Swish activation function \cite{ramachandran2017searching}. For TFN and the SE(3) Transformer we swept over different number of vector types and features and chose those that provided the best performance. Further implementation details are provided in Appendix \ref{sec:appendix_implementation_dynamical}. A Linear model that simply considers the motion equation $\rmp^{(t)} = \rmp^{(0)} + \rmv^{(0)}t$ is also included as a baseline. We also provide the average forward pass time in seconds for each of the models for a batch of 100 samples in a GTX 1080 Ti GPU.
%\textbf{Preserving equivariance to $\rmv_i$}: In this experiment we want to input some initial conditions $\rmp_i$ and $\rmv_i$. Inputting $\rmp_i$ is straightforward, it can be directly inputted to the first line of equation \ref{eq:proposed_model} as the equivariant coordinates $\rmx_i^{(0)}$. Regarding the initial conditions $\rmv_i$, it would also be benefitial to also preserve equivariance to rotations ans translations on them. To achieve this we preserve a change of basis that keeps the coordinates $\mathbf{v}_i$ equivariant to rotations and translation. This change of basis can be applicable to any other vector whose equivariance we want to preserve and it is not restricted to only velocity.

%The procedure is very simple. We just project each particle's velocity $\rmv_i$ from each node $i$, into the normalized vectors $(x_j - x_i)$ associated to each of its neighbors $j \in \mathcal{N}(i)$. The operation will be as follows:
%\begin{equation}
%    v_{ij} = \rmv_i \cdot \frac{\x_j - %\x_i}{\lVert \x_j - \x_i\rVert}
%\end{equation}
%The scalar value $v_{ij}$ is the projection of the vector $\rmv_i$ on the base $\frac{\x_j - \x_i}{\lVert \x_j - \x_i\rVert}$. We input these scalar values as an attribute $e_{ij}$ in equation \ref{eq:proposed_model} for each edge. The value of these scalar will be invariant to rotations and translations on the set of particles (prove it in the appendix).


\begin{table}[h] 
  \centering
  \begin{tabular}{lcc}
  \toprule
    Method & MSE & Forward time (s)  \\
    \midrule
    Linear & 0.0819 & .0001  \\
       SE(3) Transformer & 0.0244 & .1346  \\ 
       Tensor Field Network & 0.0155 & .0343  \\ 
        Graph Neural Network &  0.0107 & .0032  \\ 
       Radial Field & 0.0104 & .0039  \\
    \textbf{EGNN} & \textbf{0.0071}  & .0062\\ 
    \bottomrule
  \end{tabular}
  \caption{Mean Squared Error for the future position estimation in the N-body system experiment, and forward time in seconds for a batch size of 100 samples running in a GTX 1080Ti GPU.}
  \label{table:n_body}
\end{table}
\vspace{-5pt}

\textbf{Results}
As shown in Table \ref{table:n_body} our model significantly outperforms the other equivariant and non-equivariant alternatives while still being efficient in terms of running time. It reduces the error with respect to the second best performing method by a $32\%$. In addition it doesn't require the computation of spherical harmonics which makes it more time efficient than Tensor Field Networks and the SE(3) Transformer.



\begin{figure}[h!]
\begin{center}
\centerline{\includegraphics[width=0.8\columnwidth]{Figures/n_body.png}}
%\vspace{-5pt}
\caption{Mean Squared Error in the N-body experiment for the Radial Field, GNN and EGNN methods when sweeping over different amounts of training data.}
\label{fig:n_body_figure}
\end{center}
\vskip -0.25in
\end{figure}


\textbf{Analysis for different number of training samples:} We want to analyze the performance of our EGNN in the small and large data regime. In the following, we report on a similar experiment as above, but instead of using 3.000 training samples we generated a new training partition of 50.000 samples and we sweep over different amounts of data from 100 to 50.000 samples. We compare the performances of our EGNN vs its non-equivariant GNN counterpart and the Radial Field algorithm. Results are presented in Figure \ref{fig:n_body_figure}. Our method outperforms both Radial Field and GNNs in the small and large data regimes. This shows the EGNN is more data efficient than GNNs since it doesn't require to generalize over rotations and translations of the data while it ensembles the flexibility of GNNs in the larger data regime. Due to its high model bias, the Radial Field algorithm performs well when data is scarce but it is unable to learn the subtleties of the dataset as we increase the training size. In summary, our EGNN benefits from both the high bias of $\En$ methods and the flexibility of GNNs.


\subsection{Graph Autoencoder} \label{sec:expriment_autoencoder}



A Graph Autoencoder can learn unsupervised representations of graphs in a continuous latent space \cite{kipf2016variational, simonovsky2018graphvae}. In this experiment section we use our EGNN to build an Equivariant Graph Autoencoder. We will explain how Graph Autoencoders can benefit from equivariance and we will show how our method outperforms standard GNN autoencoders in the provided datasets. This problem is particularly interesting since the embedding space can be scaled to larger dimensions and is not limited to a 3 dimensional Euclidean space.

Similarly to the work of \cite{kipf2016variational} further extended by section 3.3 in \cite{liu2019graph}, our graph auto-encoder $\rmz = q(\mathcal{G})$ embeds a graph $\mathcal{G}$ into a set of latent nodes $\rmz = \{\rmz_1, \dots \rmz_M \} \in \mathbb{R}^{M \times n}$, where $M$ is the number of nodes and $n$ the embedding size per node. Notice this may reduce the memory complexity to store the graphs from $O(M^2)$ to $O(Mn)$ where $n$ may depend on $M$ for a certain approximation error tolerance. This differs from the variational autoencoder proposed in \cite{simonovsky2018graphvae} which embeds the graph in a single vector $\rmz \in \mathbb{R}^K$, which causes the reconstruction to be computationally very expensive since the nodes of the decoded graph have to be matched again to the ground truth. In addition to the introduced graph generation and representation learning methods, it is worth it mentioning that in the context of graph compression other methods \cite{candes2009exact} can be used.

More specifically, we will compare our Equivariant Graph Auto-Encoder in the task presented in \cite{liu2019graph} where a graph $\mathcal{G} = (\mathcal{V}, \mathcal{E})$ with node features $H \in \mathbb{R}^{M \times \text{nf}}$ and adjacency matrix $A \in \{0, 1\}^{M \times M}$ is embedded into a latent space $\rmz = q(H, A) \in \mathbb{R}^{M \times n}$. Following \cite{kipf2016variational, liu2019graph}, we are only interested in reconstructing the adjacency matrix $A$ since the datasets we will work with do not contain node features. The decoder $g(\cdot)$ proposed by \cite{liu2019graph} takes as input the embedding space $\rmz$ and outputs the reconstructed adjacency matrix $\hat{A} = g(\rmz)$, this decoder function is defined as follows:
\begin{equation} \label{eq:graph_decoder}
    \hat{A}_{ij} = g_e(\rmz_i, \rmz_j)=\frac{1}{1 + \mathrm{exp}(
w\left\|\rmz_{i}- \rmz_{j}\right\|^{2} + b
)}
\end{equation}

Where $w$ and $b$ are its only learnable parameters and $g_e(\cdot)$ is the decoder edge function applied to every pair of node embeddings. It reflects that edge probabilities will depend on the relative distances among node embeddings. The training loss is defined as the binary cross entropy between the estimated and the ground truth edges $\mathcal{L} = \sum_{ij}\mathrm{BCE}(\hat{A}_{ij}, A_{ij})$.


\textbf{The symmetry problem:} The above stated autoencoder may seem straightforward to implement at first sight but in some cases there is a strong limitation regarding the symmetry of the graph. Graph Neural Networks are convolutions on the edges and nodes of a graph, i.e. the same function is applied to all edges and to all nodes. In some graphs (e.g. those defined only by its adjacency matrix) we may not have input features in the nodes, and for that reason the difference among nodes relies only on their edges or neighborhood topology. Therefore, if the neighborhood of two nodes is exactly the same, their encoded embeddings will be the same too. A clear example of this is a cycle graph (an example of a 4 nodes cycle graph is provided in Figure \ref{fig:symmetric_cycle_graph}). When running a Graph Neural Network encoder on a node featureless cycle graph, we will obtain the exact same embedding for each of the nodes, which makes it impossible to reconstruct the edges of the original graph from the node embeddings. The cycle graph is a severe example where all nodes have the exact same neighborhood topology but these symmetries can be present in different ways for other graphs with different edge distributions or even when including node features if these are not unique.

\begin{figure}[h]
\begin{center}
\centerline{\includegraphics[width=0.7\columnwidth]{Figures/on_breakin_symmetry.png}}
\caption{Visual representation of a Graph Autoencoder for a 4 nodes cycle graph. The bottom row illustrates that adding noise at the input graph breaks the symmetry of the embedding allowing the reconstruction of the adjacency matrix.}
\label{fig:symmetric_cycle_graph}
\end{center}
\vskip -0.2in
\end{figure}




  \begin{figure*}[t]
    \centering
    \vspace{-.3cm}
    \begin{minipage}[c]{.59\textwidth}
    \begin{tabular}{lcccccc}
    \toprule
     & \multicolumn{3}{c}{Community Small} &   \multicolumn{3}{c}{Erdos\&Renyi}\\
    Encoder & BCE & \% Error & F1 & BCE & \% Error & F1 \\
    \midrule
    Baseline & - & 31.79 & .0000 & - & 25.13 & 0.000    \\
    GNN & 6.75 & 1.29 & 0.980 & 14.15 & 4.62 & 0.907  \\
    Noise-GNN & 3.32 & 0.44 & 0.993 & 4.56 & 1.25 & 0.975  \\
    %Noise-GNN*  & - & 0.57  & - & 3.25\\
    Radial Field & 9.22 & 1.19 & 0.981 & 6.78 & 1.63 & 0.968 \\
    EGNN & \textbf{2.14} & \textbf{0.06} & \textbf{0.999} & \textbf{1.65} & \textbf{0.11} & \textbf{0.998}  \\
    \bottomrule
    \end{tabular}
    \end{minipage}\begin{minipage}[c]{.4\textwidth}\vspace{.3cm}
    \centering
    \includegraphics[width=0.99\textwidth]{Figures/sweep_pe.png}
    \end{minipage}
    \captionlistentry[figure]{}
    %\captionsetup{labelformat=andtable}
    \vspace{-.2cm}
    \caption{In the Table at the left we report the Binary Cross Entropy, \% Error and F1 scores for the test partition on the Graph Autoencoding experiment in the Community Small and Erdos\&Renyi datasets. In the Figure at the right, we report the F1 score when overfitting a training partition of 100 samples in the Erdos\&Renyi dataset for different values of sparsity $p_e$. The GNN is not able to successfully auto-encode sparse graphs (small $p_e$ values) for the Erdos\&Renyi dataset even when training and testing on the same small subset.}
    \vspace{-.2cm}
    \label{table:autoencoder_results}
  \end{figure*}


An ad-hoc method to break the symmetry of the graph is introduced by \cite{liu2019graph}. This method introduces noise sampled from a Gaussian distribution into the input node features of the graph $\rmh_i^{0} \sim \mathcal{N}(\mathbf{0}, \sigma\mathbf{I})$. This noise allows different representations for all node embeddings and as a result the graph can be decoded again, but it comes with a drawback, the network has to generalize over the new introduced noise distribution. Our Equivariant Graph Autoencoder will remain translation and rotation equivariant to this sampled noise which we find makes the generalization much easier. Another way of looking at this is considering the sampled noise makes the node representations go from structural to positional  \cite{srinivasan2019equivalence} where $\En$ equivariance may be beneficial. In our case we will simply input this noise as the input coordinates $\rmx^{0} \sim \mathcal{N}(\mathbf{0}, \sigma\mathbf{I}) \in \mathbb{R}^{M \times n}$ of our EGNN which will output an equivariant transformation of them $\rmx^L$, this output will be used as the embedding of the graph (i.e. $\rmz = \rmx^L$) which is the input to the decoder from Equation \ref{eq:graph_decoder}.




\textbf{Dataset:} We generated community-small graphs \cite{you2018graphrnn, liu2019graph} by running the original code from \cite{you2018graphrnn}. These graphs contain $12\leq M \leq20$ nodes. We also generated a second dataset using the Erdos\&Renyi generative model \cite{bollobas2001random} sampling random graphs with an initial number of $7\leq M \leq16$ nodes and edge probability $p_e=0.25$. We sampled $5.000$ graphs for training, $500$ for validation and $500$ for test for both datasets. Each graph is defined as and adjacency matrix $A \in \{0, 1\}^{M \times M}$.

\textbf{Implementation details:} Our Equivariant Graph Auto-Encoder is composed of an EGNN encoder followed by the decoder from Equation \ref{eq:graph_decoder}. The graph edges $A_{ij}$ are input as edge attributes $a_{ij}$ in Equation \ref{eq:method_edge}. The noise used to break the symmetry is input as the coordinates $\rmx^0 \sim \mathcal{N(\mathbf{0}, \sigma\mathbf{I})} \in \mathbb{R}^{M \times n}$ in the first layer and $\rmh^0$ is initialized as ones since we are working with featureless graphs. As mentioned before, the encoder outputs an equivariant transformation on the coordinates which is the graph embedding and input to the decoder $\rmz = \rmx^L \in \mathbb{R}^{M\times n}$. We use $n=8$ dimensions for the embedding space. We compare the EGNN to its GNN cousin, we also compare to Noise-GNN which is an adaptation of our GNN to match the setting from \cite{liu2019graph}, and we also include the Radial Field algorithm as an additional baseline. All four models have 4 layers, 64 features for the hidden layers, the Swish activation function as a non-linearity and they were all trained for 100 epochs using the Adam optimizer and learning rate $10^{-4}$. More details are provided in Appendix \ref{sec:appendix_implementation_graph_autoencoders}. Since the number of nodes is larger than the number of layers, the receptive field of a GNN may not comprise the whole graph which can make the comparison unfair with our EGNN. To avoid this limitation, all models exchange messages among all nodes and the edge information is provided as edge attributes $a_{ij} = A_{ij}$ in all of them.


\textbf{Results:} In the table from Figure \ref{table:autoencoder_results} we report the Binary Cross Entropy loss between the estimated and ground truth edges, the \% Error which is defined as the percentage of wrong predicted edges with respect to the total amount of potential edges, and the F1 score of the edge classification, all numbers refer to the test partition. We also include a "Baseline" that predicts all edges as missing $\hat{A}_{ij}=0$. The standard GNN seems to suffer from the symmetry problem and provides the worst performance. When introducing noise (Noise-GNN), both the loss and the error decrease showing that it is actually useful to add noise to the input nodes. Finally, our EGNN remains $\En$ equivariant to this noise distribution and provides the best reconstruction with a $0.11\%$ error in the Erdos\&Renyi dataset and close to optimal $0.06\%$ in the Community Small dataset. A further analysis of the reconstruction error for different $n$ embedding sizes is reported in Appendix \ref{sec:appendix_graph_autoencoder}. 


\begin{table*}[th]
  \centering
  \begin{tabular}{l c c c c c c c c c c c c}
  \toprule
    Task & $\alpha$ & $\Delta \varepsilon$ & $\varepsilon_{\mathrm{HOMO}}$ & $\varepsilon_{\mathrm{LUMO}}$ & $\mu$ & $C_{\nu}$ & $G$ & $H$ & $R^2$ & $U$ & $U_0$ & ZPVE \\
    Units & bohr$^3$ & meV & meV & meV & D & cal/mol K & meV & meV & bohr$^3$ & meV & meV & meV \\
    \midrule
    %WaveScatt & .160 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 \\
    NMP & .092 & 69 & 43 & 38 & .030 & .040 & 19 & 17 & .180 & 20 & 20 & 1.50 \\
    Schnet & .235 & 63 & 41 & 34 & .033 & .033 & 14 & 14 & .073 & 19 & 14 & 1.70 \\
    Cormorant & .085 & 61 & 34 & 38 & .038 & .026 & 20 & 21 & .961 & 21 & 22 & 2.03  \\
    L1Net & .088 & 68 & 46 & 35 & .043 & .031 & 14 & 14 & .354 & 14 & 13 &  1.56\\
    
    LieConv & .084 & 49 & 30 & 25 & .032 & .038 & 22 & 24 & .800 & 19 & 19 & 2.28 \\
    DimeNet++* & .044 & 33 & 25 & 20 & .030 & .023 & 8 & 7 & .331 & 6 & 6 & 1.21  \\
    TFN & .223 & 58 & 40 & 38 & .064 & .101 & - & - & - & - & - & - \\
    SE(3)-Tr. & .142 & 53 & 35 & 33 & .051 & .054 & - & - & - & - & - & -  \\
    \midrule
    EGNN & .071  & 48 & 29 & 25 & .029 & .031 & 12 & 12 & .106 & 12 & 11 & 1.55  \\
    \bottomrule
  \end{tabular}
  \caption{Mean Absolute Error for the molecular property prediction benchmark in QM9 dataset. *DimeNet++ uses slightly different train/val/test partitions than the other papers listed here.}
  \label{tab:qm9}
\end{table*}


\textbf{Overfitting the training set:} We explained the symmetry problem and we showed the EGNN outperforms other methods in the given datasets. Although we observed that adding noise to the GNN improves the results, it is difficult to exactly measure the impact of the symmetry limitation in these results independent from other factors such as generalization from the training to the test set. In this section we conduct an experiment where we train the different models in a subset of 100 Erdos\&Renyi graphs and embedding size $n=16$ with the aim to overfit the data. We evaluate the methods on the training data. In this experiment the GNN is unable to fit the training data properly while the EGNN can achieve perfect reconstruction and Noise-GNN close to perfect. We sweep over different $p_e$ sparsity values from $0.1$ to $0.9$ since the symmetry limitation is more present in very sparse or very dense graphs. We report the F1 scores of this experiment in the right plot of Figure \ref{table:autoencoder_results}.


In this experiment we showed that $\En$ equivariance improves performance when embedding graphs in a continuous space as a set of nodes in dimension $n$. Even though this is a simple reconstruction task, we think this can be a useful step towards generating graphs or molecules where often graphs (i.e. edges) are decoded as pairwise distances or similarities between nodes e.g. \cite{kipf2016variational, liu2019graph, grover2019graphite}, and these metrics (e.g. eq. \ref{eq:graph_decoder}) are $\En$ invariant. Additionally this experiment also showed that our method can successfully perform in a $\En$ equivariant task for higher dimensional spaces where $n>3$.




\subsection{Molecular data | QM9}
The QM9 dataset \cite{ramakrishnan2014quantum} has become a standard in machine learning as a chemical property prediction task. The QM9 dataset consists of small molecules represented as a set of atoms (up to 29 atoms per molecule), each atom having a 3D position associated and a five dimensional one-hot node embedding that describe the atom type (H, C, N, O, F). The dataset labels are a variety of chemical properties for each of the molecules which are estimated through regression. These properties are invariant to translations, rotations and reflections on the atom positions.
Therefore those models that are E(3) invariant are highly suitable for this task. 

We imported the dataset partitions from \cite{anderson2019cormorant}, 100K molecules for training, 18K for validation and 13K for testing. A variety of 12 chemical properties were estimated per molecule. We optimized and report the Mean Absolute Error between predictions and ground truth.

\textbf{Implementation details:} Our EGNN receives as input the 3D coordinate locations of each atom which are provided as $\rmx_i^0$ in Equation \ref{eq:method_edge} and an embedding of the atom properties which is provided as input node features $\rmh_i^0$.  Since this is an invariant task and also $\rmx^0$ positions are static, there is no need to update the particle's position $\rmx$ by running Equation \ref{eq:method_coords} as we did in previous experiments. Consequently, we tried both manners and we didn't notice any improvement by updating $\rmx$. When not updating the particle's position (i.e. skipping Equation \ref{eq:method_coords}), our model becomes $\mathrm{E}(n)$ invariant, which is analogous to a standard GNN where all relative squared norms between pairs of points $\| \rmx_i - \rmx_j \|^2$ are inputted to the edge operation (eq. \ref{eq:method_edge}). Additionally, since we are not provided with an adjacency matrix and molecules can scale up to 29 nodes, we use the extension of our model from Section \ref{sec:edges_inference} that infers a soft estimation of the edges. Our EGNN network consists of 7 layers, 128 features per hidden layer and the Swish activation function as a non-linearity. A sum-pooling operation preceded and followed by two layers MLPs maps all the node embeddings $\rmh^{L}$ from the output of the EGNN to the estimated property value. Further implementation details are reported in Appendix. \ref{sec:appendix_implementation}. We compare to NMP \cite{gilmer2017neural}, Schnet \cite{schutt2017schnet}, Cormorant \cite{anderson2019cormorant}, L1Net \cite{miller2020relevance}, LieConv \cite{finzi2020generalizing}, DimeNet++ \cite{klicpera2020fast}, TFN \cite{thomas2018tensor} and SE(3)-Tr. \cite{fuchs2020se}.

\textbf{Results} are presented in Table \ref{tab:qm9}. Our method reports very competitive results in all property prediction tasks while remaining relatively simple, i.e. not introducing higher order representations, angles or spherical harmonics. %state of the art in 9 out of 12 property predictions, and it is the second best performing method for the remaining 3 properties. 
Perhaps, surprisingly, we outperform other equivariant networks that consider higher order representations while in this task, we are only using type-0 representations (i.e. relative distances) to define the geometry of the molecules. In Appendix \ref{appendix:invariant_features} we prove that when only positional information is given (i.e. no velocity or higher order type features), then the geometry is completely defined by the norms in-between points up to $\En$-transformations, in other words, if two collections of points separated by $\En$ transformations are considered to be identical, then the relative norms between points is a unique identifier of the collection.


==> E(n) Equivariant Graph Neural Networks _ ICML 2021/sections/index.tex <==
\section{Index}

\begin{enumerate}
    \item Introduction
    \item Equivariance
    \item Our method
    \item Related Work: compare our equations with other methods.
    \item Exp: N-body system
    \begin{itemize}
        \item Compare GNN (kipf), Kholer, SE(3), Ours. (if it is possible add TFN and LieConv
        \item Curves as we increase the number of training samples
        \item Curves as we perform data augmentation
    \end{itemize}
    \item On breaking the symmetry example
    \item Graph Autoencoder
        \begin{itemize}
            \item Compare models GNN (Thomas), GNN-Noise (GNF), SNE, Kholer, \textbf{EGNN}
            \item Compare on Community dataset, EGO dataset and Erdos\&renyi generated graphs
            \item Show training curves
            \item Sweep different embedding sizes K
            \item Sweep different \# inference iterations.
        \end{itemize}
    \item Exp: Invariant classification task, QM9 dataset, provide competitive results.
    \item Towards geometrically generating graphs: show the potential of our model to generate 3d molecules with a very simple experiment.
    
\end{enumerate}

==> E(n) Equivariant Graph Neural Networks _ ICML 2021/sections/introduction.tex <==
\begin{figure}
\begin{center}
\includegraphics[width=0.99\columnwidth]{Figures/overview_equivariance.pdf}
\caption{Example of rotation equivariance on a graph with a graph neural network $\phi$}
\label{fig:overview_equivariance}
\end{center}
\end{figure}
\vspace{-5pt}

\section{Introduction}
% Equivariance is cool
Although deep learning has largely replaced hand-crafted features, many advances are critically dependent on inductive biases in deep neural networks. An effective method to restrict neural networks to relevant functions is to exploit the \textit{symmetry} of problems by enforcing equivariance with respect to transformations from a certain symmetry group. Notable examples are translation equivariance in Convolutional Neural Networks and permutation equivariance in Graph Neural Networks \cite{bruna2013spectral, defferrard2016convolutional, kipf2016semi}. 

% Still needs editing.
Many problems exhibit 3D translation and rotation symmetries. Some examples are point clouds \cite{uy2019revisiting}, 3D molecular structures \cite{ramakrishnan2014quantum} or N-body particle simulations \cite{kipf2018neural}. The group corresponding to these symmetries is named the Euclidean group: SE(3) or when reflections are included E(3). It is often desired that predictions on these tasks are either equivariant or invariant with respect to E(3) transformations.

% SE(3) equivariance is cool, studies focus on higher types representations.
Recently, various forms and methods to achieve E(3) or SE(3) equivariance have been proposed \cite{thomas2018tensor, fuchs2020se, finzi2020generalizing, kohler2020equivariant_icml}. Many of these works achieve innovations in studying types of higher-order representations for intermediate network layers. However, the transformations for these higher-order representations require coefficients or approximations that can be expensive to compute. Additionally, in practice for many types of data the inputs and outputs are restricted to scalar values (for instance temperature or energy, referred to as type-$0$ in literature) and 3d vectors (for instance velocity or momentum, referred to as type-$1$ in literature). 
% In \cite{thomas2018tensor,fuchs2020se} the higher type representations are transformed according to the spherical harmonics which need to be recomputed for each datapoint and can be expensive.


% A big part of the current deep learning advances come from inductive baises. A successful way to include inductive biases in deep learning models is by exploiting the symmetries of the data using equivariant functions. Equivariance has proven his success in a variety of applications, for example, Convolutional Neural Networks (CNNs) are translation equivariant, which means that a translation of the input image corresponds to an equivalent translation of the output feature map. This discards the need to do data augmentation reducing the computating resouces in terms of training time and model capacity. Equivariance can also be found in other successful cases like permutation equivariance in Graph Neural Networks 

% Other directions


In this work we present a new architecture that is translation, rotation and reflection equivariant ($\En$), and permutation equivariant with respect to an input set of points. Our model is simpler than previous methods in that it does not require the spherical harmonics as in \cite{thomas2018tensor, fuchs2020se} while it can still achieve competitive or better results. In addition, equivariance in our model is not limited to the 3-dimensional space and can be scaled to larger dimensional spaces without a significant increase in computation. 

We evaluate our method in modelling dynamical systems, representation learning in graph autoencoders and predicting molecular properties in the QM9 dataset. Our method reports the best or very competitive performance in all three experiments.

==> E(n) Equivariant Graph Neural Networks _ ICML 2021/sections/model.tex <==
\section{Equivariant Graph Neural Networks} 
% \label{sec:method}

% \subsection{}yes
\label{sec:method_main}
In this section we present Equivariant Graph Neural Networks (EGNNs). Following the notation from background Section \ref{sec:background_gnn}, we consider a graph $\mathcal{G} = (\mathcal{V},\mathcal{E})$ with nodes $v_i \in \mathcal{V}$ and edges $e_{ij} \in \mathcal{E}$. In addition to the feature node embeddings $\rmh_i \in \mathbb{R}^{\text{nf}}$ we now also consider a $n$-dimensional coordinate $\rmx_i \in  \mathbb{R}^{\text{n}}$ associated with each of the graph nodes. Our model will preserve equivariance to rotations and translations on these set of coordinates $\rmx_i$ and it will also preserve equivariance to permutations on the set of nodes $\mathcal{V}$ in the same fashion as GNNs.

%Although the dimensionality $d$ of $\rmx_i$ usually takes values 2 or 3 for most physic scenarios, our model can scale to larger dimensions without a significant increase in computation.

%Our equivariant graph convlutional layer takes as We want our model to be translation and rotation equivariant to $\rmx_i$ and equivariant to permutations of the nodes $v_i$. Following we introduce the equations of our algorithm which despite of its simplicity fulfill the proposed equivariant constraints, scale to large d-dimensional and still provide very strong results. 

Our Equivariant Graph Convolutional Layer (EGCL) takes as input the set of node embeddings $\rmh^l =\{\rmh_0^l, \dots, \rmh_{M-1}^l\}$, coordinate embeddings $\rmx^l =\{\rmx_0^l, \dots, \rmx_{M-1}^l\} $ and edge information $\mathcal{E}=(e_{ij})$ and outputs a transformation on $\rmh^{l+1}$ and $\rmx^{l+1}$. Concisely: $\rmh^{l+1}, \rmx^{l+1} = \text{EGCL}[\rmh^{l}, \rmx^{l}, \mathcal{E}]$. The equations that define this layer are the following:
\begin{align}\label{eq:method_edge}
\rmm_{ij} &=\phi_{e}\left(\rmh_{i}^{l}, \rmh_{j}^{l},\left\|\rmx_{i}^{l}-\rmx_{j}^{l}\right\|^{2}, a_{i j}\right) \\ \label{eq:method_coords}
\rmx_{i}^{l+1} &=\rmx_{i}^{l}+ C\sum_{j \neq i}\left(\rmx_{i}^{l}-\rmx_{j}^{l}\right) \phi_{x}\left(\rmm_{ij}\right) \\
 \label{eq:method_agg}
\rmm_{i} &=\sum_{j \neq i} \rmm_{ij} \\ 
\label{eq:method_node}
\rmh_{i}^{l+1} &=\phi_{h}\left(\rmh_{i}^l, \rmm_{i}\right)
\end{align}

% \begin{equation}
% \begin{aligned}\label{eq:proposed_model}
% \mathbf{m}_{i, j} &=\phi_{e}\left(\mathbf{h}_{i}^{l}, \mathbf{h}_{j}^{l},\left\|\mathbf{x}_{i}^{l}-\mathbf{x}_{j}^{l}\right\|^{2}, \left\|\mathbf{v}_{i}^{l}-\mathbf{v}_{j}^{l}\right\|^{2}, e_{i j}\right) \\
% \mathbf{x}_{i}^{l+1} &=\mathbf{x}_{i}^{l}+\sum_{j \neq i}\left(\mathbf{x}_{i}^{l}-\mathbf{x}_{j}^{l}\right) \phi_{x}\left(\mathbf{m}_{i, j}\right) +\sum_{j \neq i}\left(\mathbf{v}_{i}^{l}-\mathbf{v}_{j}^{l}\right) \phi_{v}\left(\mathbf{m}_{i, j}\right) \\
% \mathbf{m}_{i} &=\sum_{j \neq i} \mathbf{m}_{i, j} \\
% \mathbf{h}_{i}^{l+1} &=\phi_{h}\left(\mathbf{h}_{i}^l, \mathbf{m}_{i}\right)
% \end{aligned}
% \end{equation}


 %\begin{equation}
 %\begin{aligned}\label{eq:proposed_model}
 %\mathbf{m}_{i, j} &=\phi_{e}\left(\mathbf{h}_{i}^{l}, \mathbf{h}_{j}^{l},\left\|\mathbf{x}_{i}^{l}-\mathbf{x}_{j}^{l}\right\|^{2}, \left\|\mathbf{v}_{i}^{l}-\mathbf{v}_{j}^{l}\right\|^{2}, e_{i j}\right) \\
 %\mathbf{m}_{i} &=\sum_{j \neq i} \mathbf{m}_{i, j} \\
 %\mathbf{v}_{i}^{l+1}&= \mathbf{v}_{i}^{l} +\sum_{j \neq i}\left(\mathbf{x}_{i}^{l}-\mathbf{x}_{j}^{l}\right) \phi_{x}\left(\mathbf{m}_{i, j}\right) \\
 %\mathbf{x}_{i}^{l+1} &=\mathbf{x}_{i}^{l}+ \mathbf{v}_i^{l+1} \phi_{v}\left(\mathbf{m}_{i}\right)\\
 %\mathbf{h}_{i}^{l+1} &=\phi_{h}\left(\mathbf{h}_{i}^l, \mathbf{m}_{i}\right)
 %\end{aligned}
 %\end{equation}
 
Notice the main differences between the above proposed method and the original Graph Neural Network from equation \ref{eq:gnn} are found in equations \ref{eq:method_edge} and \ref{eq:method_coords}. In equation \ref{eq:method_edge} we now input the relative squared distance between two coordinates $\|\mathbf{x}_{i}^{l}-\mathbf{x}_{j}^{l}\|^{2}$ into the edge operation $\phi_e$. The embeddings $\rmh_i^l$, $\rmh_j^l$, and the edge attributes $a_{ij}$ are also provided as input to the edge operation as in the GNN case. In our case the edge attributes will incorporate the edge values $a_{ij} = e_{ij}$, but they can also include additional edge information.

In Equation \ref{eq:method_coords} we update the position of each particle $\rmx_i$ as a vector field in a radial direction. In other words, the position of each particle $\rmx_i $ is updated by the weighted sum of all relative differences $(\rmx_i - \rmx_j)_{\forall j}$. The weights of this sum are provided as the output of the function $\phi_x: \mathbb{R}^{\text{nf}} \rightarrow \mathbb{R}^1$ that takes as input the edge embedding $\rmm_{ij}$ from the previous edge operation and outputs a scalar value. $C$ is chosen to be $1/(M-1)$, which divides the sum by its number of elements. This equation is the main difference of our model compared to standard GNNs and it is the reason why equivariances 1, 2 are preserved (proof in Appendix \ref{sec:appendix_equiv_proof}). Despite its simplicity, this equivariant operation is very flexible since the embedding $\rmm_{ij}$ can carry information from the whole graph and not only from the given edge $e_{ij}$. 

Finally, equations \ref{eq:method_agg} and \ref{eq:method_node} follow the same updates than standard GNNs. Equation \ref{eq:method_agg} is the aggregation step, in this work we choose to aggregate messages from all other nodes $j\neq i$, but we could limit the message exchange to a given neighborhood $j \in \mathcal{N}(i)$ if desired in both equations \ref{eq:method_agg} and \ref{eq:method_coords}. Equation \ref{eq:method_node} performs the node operation $\phi_h$ which takes as input the aggregated messages $\rmm_i$, the node emedding $\rmh_i^{l}$ and outputs the updated node embedding $\rmh_i^{l+1}$.




%In the first line we input the relative squared distance between two coordinates $\left\|\mathbf{x}_{i}^{l}-\mathbf{x}_{j}^{l}\right\|^{2}$ into the edge operation. The distance between two particles is invariant to rotations and translations on the set of particles, therefore, the output messages $\mathbf{m}_{ij}$ also remain invariant to translations and rotations on $X$, finally $H$ remains invariant too since it is updated from the messages $\mathbf{m}_{ij}$ that were already invariant. In the second line of equation \ref{eq:proposed_model}, the coordinates $\rmx_i$ are updated, the function $\phi_x$ takes as input the message $\rmm_{ij}$ which is invariant to rotations and translations on $\rmx_i$ and otuputs a scalar value. The coordinates $\rmx$ are updated as a weighted sum of their relative differences, this operation is equivariant to translations and rotations on $\rmx_i$, i.e. translating and rotating $\rmx^{l}$ will imply an equivalent translation and rotation on $\rmx^{l+1}$.

\subsection{Analysis on E(n) equivariance} \label{sec:equivariance_proof}
In this section we analyze the equivariance properties of our model for $E(3)$ symmetries (i.e. properties 1 and 2 stated in section \ref{sec:background_equivariance}). In other words, our model should be translation equivariant on $\rmx$ for any translation vector $g \in \mathbb{R}^n$ and it should also be rotation and reflection equivariant on $\rmx$ for any orthogonal matrix $Q \in \mathbb{R}^{n \times n}$. More formally our model satisfies:
%
\begin{equation*}
    Q\rmx^{l+1} + g, \rmh^{l+1}  = \mathrm{EGCL}(Q\rmx^l + g, \rmh^l)
\end{equation*}
%
We provide a formal proof of this in Appendix \ref{sec:appendix_equiv_proof}. Intuitively, let's consider a $\rmh^l$ feature which is already $\En$ invariant, then we can see that the resultant edge embedding $\rmm_{ij}$ from Equation \ref{eq:method_edge} will also be $\En$ invariant, because in addition to $\rmh^l$, it only depends on squared distances $\|\rmx_{i}^l-\rmx_{j}^l\|^{2}$, which are $\En$ invariant. Next, Equation \ref{eq:method_coords} computes $\rmx^{l+1}_i$ by a weighted sum of differences $(\rmx_i - \rmx_j)$ which is added to $\rmx_i$, this transforms as a type-1 vector and preserves equivariance (see Appendix \ref{sec:appendix_equiv_proof}). Finally the last two equations \ref{eq:method_agg} and \ref{eq:method_node} that generate the next layer node-embeddings $\rmh^{l+1}$ remain $\En$ invariant since they only depend on $\rmh^l$ and $\rmm_{ij}$ which, as we saw above, are $\En$ invariant. Therefore the output $\rmh^{l+1}$ is $\En$ invariant and $\rmx^{l+1}$ is $\En$ equivariant to $\rmx^{l}$. Inductively, a composition of $\mathrm{EGCL}$s will also be equivariant.

\subsection{Extending EGNNs for vector type representations} \label{sec:method_velocity}
In this section we propose a slight modification to the presented method such that we explicitly keep track of the particle's momentum. In some scenarios this can be useful not only to obtain an estimate of the particle's velocity at every layer but also to provide an initial velocity value in those cases where it is not 0. We can include momentum to our proposed method by just replacing Equation \ref{eq:method_coords} of our model with the following equation:
\begin{equation} \label{eq:egnn_velocity}
    \begin{aligned}
     %\mathbf{v}_{i}^{l+1}&= \phi_{v}\left(\rmh_{i}^l\right)\rmv_{i}^{l} + C\sum_{j \neq i}\left(\mathbf{x}_{i}^{l}-\mathbf{x}_{j}^{l}\right) \phi_{x}\left(\mathbf{m}_{ij}\right) \\ 
    \mathbf{v}_{i}^{l+1}&= \phi_{v}\left(\rmh_{i}^l\right)\rmv_{i}^\text{init} + C\sum_{j \neq i}\left(\mathbf{x}_{i}^{l}-\mathbf{x}_{j}^{l}\right) \phi_{x}\left(\mathbf{m}_{ij}\right) \\
 \rmx_{i}^{l+1} &=\mathbf{x}_{i}^{l}+ \mathbf{v}_i^{l+1}
    \end{aligned}
\end{equation}
Note that this extends the EGCL layer as $\rmh^{l+1}, \rmx^{l+1}, \rmv^{l+1} = \text{EGCL}[\rmh^{l}, \rmx^{l}, \rmv^{\text{init}}, \mathcal{E}]$. The only difference is that now we broke down the coordinate update (eq. \ref{eq:method_coords}) in two steps, first we compute the velocity $\rmv^{l+1}_i$ and then we use this velocity to update the position $\rmx^l_i$. The initial velocity $\rmv^{\text{init}}_i$ is scaled by a new function $\phi_v: \mathbb{R}^N \rightarrow \mathbb{R}^1$ that maps the node embedding $\rmh_i^l$ to a scalar value. Notice that if the initial velocity is set to zero (${\rmv}^{\text{init}}_i = 0$), both equations \ref{eq:method_coords} and \ref{eq:egnn_velocity} become exactly the same. We proof the equivariance of this variant of the model in Appendix \ref{sec:appendix_equiv_proof_velocity}. This variant is used in experiment \ref{sec:experiment_n_body} where we provide the initial velocity of the system, and predict a relative position change.


\begin{table*}[t] \tiny
  \centering
  \begin{tabular}{|l | c | c | c | c | c | c}
  \toprule
     & GNN & Radial Field & TFN & Schnet  & EGNN \\
    \midrule
    \multirow{2}*{Edge} & 
    \multirow{2}*{$\rmm_{ij} = \phi_e(\rmh_i^l, \rmh_j^l, a_{ij})$} &
    \multirow{2}*{$\rmm_{ij} = \phi_{\text{rf}}(\|\rmr_{ij}^{l}\|) \rmr_{ij}^{l}$} &
    \multirow{2}*{$\rmm_{ij} =  \sum_{k}\mathbf{W}^{lk}\rmr_{ji}^{l}\rmh_i^{lk}$} &
    \multirow{2}*{$\rmm_{ij}=\phi_{\text{cf}}(\|\rmr_{ij}^{l}\|) \phi_\text{s}(\rmh_{j}^{l})$ } & 
    $\mathbf{m}_{ij} =\phi_{e}(\mathbf{h}_{i}^{l}, \mathbf{h}_{j}^{l},\|\rmr_{ij}^{l}\|^{2}, a_{i j})$   \\
    & &  & & & $\hat{\rmm}_{ij} = \rmr_{ij}^{l}\phi_x(\rmm_{ij})$  \\
    \midrule
    \multirow{2}*{Agg}. &
    \multirow{2}*{$\summessages$} &
    \multirow{2}*{$\summessagesb$} &
    \multirow{2}*{$\summessagesb$} &
    \multirow{2}*{$\summessagesb$} &
    $\summessagesb$ \\
     & & & & &
     $\hat{\rmm}_i = C\sum_{j \neq i} \hat{\rmm}_{ij}$ \\
    \midrule
    \multirow{2}*{Node} &
    \multirow{2}*{$\rmh_i^{l+1} = \phi_h(\rmh_i^l, \rmm_i)$} &
    \multirow{2}*{$\rmx_i^{l+1} = \rmx_i^{l} + \rmm_i$} &
    \multirow{2}*{$\rmh_i^{l+1} = w^{ll}\rmh_i^{l} + \rmm_i$} &
    \multirow{2}*{$\rmh_i^{l+1} = \phi_h(\rmh_i^l, \rmm_i)$} &
    $\mathbf{h}_{i}^{l+1} =\phi_{h}\left(\mathbf{h}_{i}^l, \mathbf{m}_{i}\right)$ \\
         &
     &
     &
     &
     &
    $\rmx_i^{l+1} = \rmx_i^{l} + \hat{\rmm}_i $  \\
    \midrule
     &
    Non-equivariant &
    $\En$-Equivariant &
    $\mathrm{SE}(3)$-Equivariant &
    $\En$-Invariant &
    $\En$-Equivariant  \\
    \bottomrule
  \end{tabular}
  \caption{Comparison over different works from the literature under the message passing framework notation. We created this table with the aim to provide a clear and simple way to compare over these different methods. The names from left to right are: Graph Neural Networks \cite{gilmer2017neural}; Radial Field from Equivariant Flows \cite{kohler2019equivariant_workshop}; Tensor Field Networks \cite{thomas2018tensor}; Schnet \cite{schutt2017schnet}; and our Equivariant Graph Neural Network. The difference between two points is written $\rmr_{ij} = (\rmx_i - \rmx_j)$.}
  \label{tab:related_work}
\end{table*}


\subsection{Inferring the edges} \label{sec:edges_inference}
Given a point cloud or a set of nodes, we may not always be provided with an adjacency matrix. In those cases we can assume a fully connected graph where all nodes exchange messages with each other $j \neq i$ as done in Equation \ref{eq:method_agg}. This fully connected approach may not scale well to large point clouds where we may want to locally limit the exchange  of messages $\rmm_i = 
   \sum_{j \in \mathcal{N}(i)}\rmm_{ij}$ to a neighborhood $\mathcal{N}(i)$ to avoid an overflow of information.

Similarly to \cite{serviansky2020set2graph, kipf2018neural}, we present a simple solution to infer the relations/edges of the graph in our model, even when they are not explicitly provided. Given a set of neighbors $\mathcal{N}(i)$ for each node $i$, we can re-write the aggregation operation from our model (eq. \ref{eq:method_agg}) in the following way:
\begin{equation}\label{eq:attention}
   \rmm_i = 
   \sum_{j \in \mathcal{N}(i)}\rmm_{ij} = \sum_{j \neq i} e_{ij}\rmm_{ij} 
\end{equation}
Where $e_{ij}$ takes value $1$ if there is an edge between nodes $(i,j)$ and $0$ otherwise. %Notice this doesn't modify yet the original equation used in our model, it is just a change in notation. 
Now we can choose to approximate the relations $e_{ij}$ with the following function $e_{ij} \approx \phi_{inf}(\rmm_{ij})$, where $\phi_{inf}: \mathbb{R}^{nf} \rightarrow [0, 1]^1$ resembles a linear layer followed by a sigmoid function that takes as input the current edge embedding and outputs a soft estimation of its edge value. This modification does not change the $\En$ properties of the model since we are only operating on the messages $\rmm_{ij}$ which are already $\En$ invariant. 
% One can think of this as an invariant soft-attention function \cite{fuchs2020se}.

==> E(n) Equivariant Graph Neural Networks _ ICML 2021/sections/related.tex <==



\section{Related Work} \label{sec:related_work}
% General equivariance romero2021group
Group equivariant neural networks have demonstrated their effectiveness in a wide variety of tasks \citep{cohen2016group,cohen2017steerable,weiler2019e2equivariant,rezende2019equivariantflows,romero2021group}.
Recently, various forms and methods to achieve E(3) or SE(3) equivariance have been proposed. \citet{thomas2018tensor, fuchs2020se} utilize the spherical harmonics to compute a basis for the transformations, which allows transformations between higher-order representations. A downside to this method is that the spherical harmonics need to be recomputed which can be expensive. Currently, an extension of this method to arbitrary dimensions is unknown. \citet{finzi2020generalizing} parametrize transformations by mapping kernels on the Lie Algebra. For this method the neural network outputs are in certain situations stochastic, which may be undesirable. \citet{horie2020isometric} proposes a set of isometric invariant and equivairant transformations for Graph Neural Networks.
\citet{kohler2019equivariant_workshop, kohler2020equivariant_icml} propose an $\En$ equivariant network to model 3D point clouds, but the method is only defined for positional data on the nodes without any feature dimensions.

Another related line of research concerns message passing algorithms on molecular data. \cite{gilmer2017neural} presented a message passing setting (or Graph Neural Network) for quantum chemistry, this method is permutation equivariant but not translation or rotation equivariant. \cite{kondor2018covariant} extends the equivariance of GNNs such that each neuron transforms in a specific way under permutations, but this extension only affects its permutation group and not translations or rotations in a geometric space. Further works \cite{schutt2017schnet, schutt2017quantum} build $\En$ invariant message passing networks by inputting the relative distances between points. \citet{klicpera2020directional, klicpera2020fast} in addition to relative distances it includes a modified message passing scheme analogous to Belief Propagation that considers angles and directional information equivariant to rotations. It also uses Bessel functions and spherical harmonics to construct and orthogonal basis. \citet{anderson2019cormorant, miller2020relevance} include $SO(3)$ equivariance in its intermediate layers for modelling the behavior and properties of molecular data. Our method is also framed as a message passing framework but in contrast to these methods it achieves $\En$ equivariance.


\subsection*{Relationship with existing methods}
 In Table \ref{tab:related_work} the EGNN equations are detailed together with some of its closest methods from the literature under the message passing notation from \cite{gilmer2017neural}. This table aims to provide a simple way to compare these different algorithms. It is structured in three main rows that describe i) the edge ii) aggregation and iii) node update operations. The GNN algorithm is the same as the previously introduced in Section \ref{sec:background_equivariance}. Our EGNN algorithm is also equivalent to the description in Section \ref{sec:method_main} but notation has been modified to match the (edge, aggregation, node) format. In all equations $\rmr_{ij}^l = (\rmx_i - \rmx_j)^l$. Notice that except the EGNN, all algorithms have the same aggregation operation and the main differences arise from the edge operation. The algorithm that we call "Radial Field" is the $\En$ equivariant update from \cite{kohler2019equivariant_workshop}. This method is $\En$ equivariant, however its main limitation is that it only operates on $\rmx$ and it doesn't propagate node features $\rmh$ among nodes. In the method $\phi_{rf}$ is modelled as an MLP. Tensor Field Networks (TFN) \cite{thomas2018tensor} instead propagate the node embeddings $\rmh$ but it uses spherical harmonics to compute its learnable weight kernel $ \mathbf{W}^{\ell k}: \mathbb{R}^{3} \rightarrow \mathbb{R}^{(2 \ell+1) \times(2 k+1)}$ which preserves $SE(3)$ equivariance but is expensive to compute an limited to the 3 dimensional space. The SE(3) Transformer \cite{fuchs2020se} (not included in this table), can be interpreted as an extension of TFN with attention. Schnet \cite{schutt2017schnet} can be interpreted as an $\En$ invariant Graph Neural Network where $\phi_{cf}$ receives as input relative distances and outputs a continuous filter convolution that multiplies the neighbor embeddings $\rmh$. Our EGNN differs from these other methods in terms that it performs two different updates in each of the table rows, one related to the embeddings $\rmh$ and another related to the coordinates $\rmx$, these two variables exchange information in the edge operation. In summary the EGNN can retain the flexibility of GNNs while remaining $\En$ equivariant as the Radial Field algorithm and without the need to compute expensive operations (i.e. spherical harmonics).

==> sections/index.tex <==
\section{Index}

\begin{enumerate}
    \item Introduction
    \item Equivariance
    \item Our method
    \item Related Work: compare our equations with other methods.
    \item Exp: N-body system
    \begin{itemize}
        \item Compare GNN (kipf), Kholer, SE(3), Ours. (if it is possible add TFN and LieConv
        \item Curves as we increase the number of training samples
        \item Curves as we perform data augmentation
    \end{itemize}
    \item On breaking the symmetry example
    \item Graph Autoencoder
        \begin{itemize}
            \item Compare models GNN (Thomas), GNN-Noise (GNF), SNE, Kholer, \textbf{EGNN}
            \item Compare on Community dataset, EGO dataset and Erdos\&renyi generated graphs
            \item Show training curves
            \item Sweep different embedding sizes K
            \item Sweep different \# inference iterations.
        \end{itemize}
    \item Exp: Invariant classification task, QM9 dataset, provide competitive results.
    \item Towards geometrically generating graphs: show the potential of our model to generate 3d molecules with a very simple experiment.
    
\end{enumerate}
